Field typing for improved recognition on heterogeneous handwritten forms

Offline handwriting recognition has undergone continuous progress over the past decades. However, existing methods are typically benchmarked on free-form text datasets that are biased towards good-quality images and handwriting styles, and homogeneous content. In this paper, we show that state-of-the-art algorithms, employing long short-term memory (LSTM) layers, do not readily generalize to real-world structured documents, such as forms, due to their highly heterogeneous and out-of-vocabulary content, and to the inherent ambiguities of this content. To address this, we propose to leverage the content type within an LSTM-based architecture. Furthermore, we introduce a procedure to generate synthetic data to train this architecture without requiring expensive manual annotations. We demonstrate the effectiveness of our approach at transcribing text on a challenging, real-world dataset of European Accident Statements.

==> paper arxiv copyrighted/related.tex <==
\section{Related work}


\subsection{Text recognition}
%--- For recognition ---
Automatic text recognition has been a longstanding goal of the document processing community, as discussed thoroughly in the survey of~\cite{eskenazi2017comprehensive}. As for many image-analysis problems, Convolutional Neural Networks~\cite{leCun_CNN} have proven highly beneficial for text recognition, starting with the simple task of classifying individual handwritten digits. These results were extended to more general characters~\cite{jaderberg2014_unconstrained}, as well as to sequence-based inputs, such as text, speech and music scores, by exploiting Markov models~\cite{plotz2009markov}. In turn, these sequential models were also replaced with artificial neural networks, in particular recurrent ones, such as the Long Short Term Memory (LSTM) of~\cite{LSTM_original}, which have proven more effective at handling long-term dependencies~\cite{graves_LSTM}. In particular, coupled with the Connectionist Temporal Classification loss, LSTMs constitute a highly-successful, alignment-free recognition method~\cite{CTC}.
Further improvements were made by using dropout within the recurrent network as a mean of regularization~\cite{MDLSTM_dropout}.


Ultimately, the current state-of-the-art architectures for both text-in-the-wild~\cite{CRNN} and handwriting~\cite{rawls2017_CNN,puigcerver_MDLSTM_vs_CNN,dutta2018_hwr} recognition combine CNN and RNN layers so as to model individual characters and sequences thereof in a single framework that can be trained in an end-to-end fashion.
This is typically achieved by using VGG-derived convolutional feature extractors followed by bi-LSTM~\cite{LSTM_original} layers. In addition, these methods usually exploit synthetic data and data augmentation to improve robustness, as well as an external language model to correct the character recognition errors. 
While most methods focus on a single language, the multilingual setting was addressed in~\cite{bluche2017gated} via a new gated convolutional feature extractor.
Note that, while convolutional extractors are the most common ones, fully-connected layers can also be employed, as demonstrated in~\cite{rawls2017_direct}. In any event, the effectiveness of these techniques has been demonstrated on academic databases only, and these databases consist of standard text lines and paragraphs. In other words, as discussed above, state-of-the-art models trained on such academic databases are ill-suited to handle structured forms with heterogeneous content. Here, we introduce an approach to handling such forms, which relies on leveraging the text type to overcome ambiguities and on generating synthetic data to avoid manual annotation.

\subsection{Synthetic data and preprocesing techniques}

Creating a synthetic dataset to compensate for the lack of annotated handwriting data has already been studied in the past. This, for instance, was the case in~\cite{synthetic_data} to generate synthetic natural scene text images and in~\cite{krishnan2016generating} to render 90k English words using a collection of handwritten fonts. In~\cite{generation_nunamaker2016tesseract}, instead of fonts, images of letters were concatenated so as to create a database used to train an OCR engine. None of these methods, however, apply to our scenario, because they generate either printed text only, without ligatures, or words from the English vocabulary, thus being ill-suited to handle OOV instances. Furthermore, they do not consider structured documents as we do here.

%--- Quality of data --- 
% The heterogeneity of the handwriting style and the quality of the image namely degraded scanned document affects the overall accuracy of the recognition \cite{smith2005text}. The classification accuracy varies depending on the degradation space of the training sample. 

When working with such documents, one needs to extract the regions containing handwritten text. This problem, however, is not the main focus of our work, and we refer the reader to~\cite{eskenazi2017comprehensive} for a comprehensive survey of the literature until 2015. More recent methods are largely divided into two classes. On one hand, there are anchor-based approaches, such as~\cite{whiteboard_classic2017}, which employs a Faster R-CNN derivative~\cite{faster_rcnn} to detect skewed text in images of whiteboards. On the other, one can make use of pixel-level segmentation, as in~\cite{whiteboard_cnn2018}, which uses SegLink~\cite{seglink}.
Alternatively, for printed text,~\cite{e2e_tables_dengel} introduces robust heuristics on top of the Tesseract OCR engine. Furthermore,~\cite{moysset_whereToStart} relies on a pair of multi-dimensional LSTMs to extract and recognize printed and handwritten text jointly.
Here, as discussed in Section~\ref{sec:method:system}, we follow an anchor-based approach, which 
we found to be effective.

